Semantic-SAM: Segment and Recognize Anything at Any Granularity

In this paper, we introduce Semantic-SAM, a universal image segmentation model to enable segment and recognize anything at any desired granularity. Our model offers two key advantages: semantic-awareness and granularity-abundance. To achieve semantic-awareness, we consolidate multiple datasets across three granularities and introduce decoupled classification for objects and parts. This allows our model to capture rich semantic information. For the multi-granularity capability, we propose a multi-choice learning scheme during training, enabling each click to generate masks at multiple levels that correspond to multiple ground-truth masks. Notably, this work represents the first attempt to jointly train a model on SA-1B, generic, and part segmentation datasets. Experimental results and visualizations demonstrate that our model successfully achieves semantic-awareness and granularity-abundance. Furthermore, combining SA-1B training with other segmentation tasks, such as panoptic and part segmentation, leads to performance improvements. We will provide code and a demo for further exploration and evaluation.

==> res/tables/generic.tex <==
% \usepackage[normalem]{ulem}
% \usepackage{multirow}
% \usepackage{colortbl}
% \usepackage{booktabs}
% \usepackage{hhline}

\begin{table*}
\caption{\textbf{Generic segmentation} of \ourmodel{} by jointly training interactive segmentation and generic segmentation. We directly evaluate the performance without finetuning. Note: ``$-$" denotes the model does not have number reported or does not have the ability for the specific task.

$\star$ means it is the test set results. The results in the bracket are trained with 1280$\times$1280 image size.
Note that the results of GLIPv2 and X-Decoder on COCO are finetuned while those of \ourmodel{} are reported without finetunning. }
\label{tab:task_transfer}
\footnotesize  \setlength{\tabcolsep}{8.0pt}
\centering
\resizebox{0.999\linewidth}{!}{
\begin{tabular}{l|c|ccc|cccc} 
\specialrule{.12em}{.1em}{.1em}
\multirow{2}{*}{Method} & \multirow{2}{*}{Type} & \multicolumn{3}{c|}{\uline{Pascal Part}} & \multicolumn{4}{c}{\uline{COCO}} \\
 & & PQ & mask AP & mIoU & PQ & mask AP & box AP & mIoU \\ 
\hline
Mask2Former (T)~\cite{cheng2022masked} & \multirow{7}{*}{Closed-set} &  63.9 & 39.1 & 80.5 & 53.2 & 43.3 & 46.1 & 63.2 \\
Mask2Former (B)~\cite{cheng2022masked} &  &53.9 & 66.1 & 42.8 & 82.7 & 56.4 & 46.3 & 49.5 & 67.1 \\
Mask2Former (L)~\cite{cheng2022masked} &  & 66.6 & 43.6 & 82.9 & 57.8 & {48.6} & 52.1 & 67.4 \\
OneFormer (L)~\cite{jain2022oneformer} &  &67.2 & 45.6 & ~83.0 & 57.9 & {48.9} & $-$ & 67.4 \\
MaskDINO (L)~\cite{li2022mask} &  & $-$ & $-$ & $-$ & 58.3 & {50.6} & 56.2 & 67.5 \\
Pano/SegFormer (B)~\cite{xie2021segformer} &  & $-$ & $-$ & $-$ & 55.4 & $-$ & $-$ & $-$ \\
kMaX-DeepLab (L)~\cite{yu2022k} &  & $-$ & $-$ & $-$ & {58.1} & $-$ & $-$ & $-$ \\ 
\hline

GLIPv2 (T)~\cite{zhang2022glipv2} & \multirow{8}{*}{Open-vocabulary} & $-$ & $-$ & $-$ & $-$ & $-\lvert$42.0$^\star$ & $-$ & $-$ \\
% GLIPv2 (B)~\cite{zhang2022glipv2} &  & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-\lvert$45.8$^\star$ & $-$ & $-$ \\
% GLIPv2 (H)~\cite{zhang2022glipv2} &  & $-$ & $-$ &$-$& $-$ & $-$ & $-$ & & $-$ & $-\lvert$48.9$^\star$ & $-$ & $-$ \\
X-Decoder (T)~\cite{zou2022generalized} &  &-&-&-&51.4 & 40.5 & 43.6 & 62.8 \\
OpenSeed (T) &  &-&-&-&
{{55.4}} & {47.6}& {52.0}& {64.0}\\
\ourmodel{} &  &-&-&-&
{{55.4}$\lvert -$} & {47.6}$\lvert -$ & {52.1}$\lvert -$ & {62.8}$\lvert -$  \\
% % X-Decoder (B) &  & 46.8 & 33.5 & $-$ & 54.6 & $-$ & $-$ & $-$ & $-\lvert$56.2 & $-\lvert$45.8 & $-$ & $-\lvert$66.0 \\
% X-Decoder (L)~\cite{zou2022generalized} &  & 49.6 & 35.8 & $-$ & 58.1 & 65.6 & 42.2 & 81.7 & $-\lvert$56.9 & $-\lvert$46.7 & $-$ & $-\lvert$67.5 \\


% {\cellcolor[rgb]{0.961,0.961,0.961}}\ourmodel{} (L) &  & {\cellcolor[rgb]{0.961,0.961,0.961}}\textbf{53.1~(53.7)} & {\cellcolor[rgb]{0.961,0.961,0.961}}\textbf{42.0~(42.6)} & {\cellcolor[rgb]{0.961,0.961,0.961}}\textbf{46.4~(46.9)} & {\cellcolor[rgb]{0.961,0.961,0.961}}\textbf{58.6~(58.4)} & {\cellcolor[rgb]{0.961,0.961,0.961}\textbf{68.9}}& {\cellcolor[rgb]{0.961,0.961,0.961}\textbf{48.5}}& {\cellcolor[rgb]{0.961,0.961,0.961}\textbf{84.5}}& {\cellcolor[rgb]{0.961,0.961,0.961}\textbf{59.5}}  & {\cellcolor[rgb]{0.961,0.961,0.961}\textbf{53.2}} & {\cellcolor[rgb]{0.961,0.961,0.961}\textbf{58.2}}& {\cellcolor[rgb]{0.961,0.961,0.961}\textbf{68.6}} \\
% \specialrule{.12em}{.1em}{.1em}
\end{tabular}
}
\end{table*}


